Synergy and Diversity in CLIP: Enhancing Performance Through Adaptive Backbone Ensembling

Contrastive Language-Image Pretraining (CLIP) stands out as a prominent method for image representation learning. Various architectures, from vision transformers (ViTs) to convolutional networks (ResNets) have been trained with CLIP to serve as general solutions to diverse vision tasks. This paper explores the differences across various CLIP-trained vision backbones. Despite using the same data and training objective, we find that these architectures have notably different representations, different classification performance across datasets, and different robustness properties to certain types of image perturbations. Our findings indicate a remarkable possible synergy across backbones by leveraging their respective strengths. In principle, classification accuracy could be improved by over 40 percentage with an informed selection of the optimal backbone per test example.Using this insight, we develop a straightforward yet powerful approach to adaptively ensemble multiple backbones. The approach uses as few as one labeled example per class to tune the adaptive combination of backbones. On a large collection of datasets, the method achieves a remarkable increase in accuracy of up to 39.1% over the best single backbone, well beyond traditional ensembles

==> figures/analysis_rnd_proj.tex <==
\begin{figure}
    \centering    
    \includegraphics[width=0.6\textwidth]{imgs/analysis_rnd_proj.pdf}
    \caption{Random projection analysis}
    \label{fig:random_proj_analysis}
\end{figure}

==> figures/improvement_vs_diversity.tex <==
\begin{figure}[b!]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/improvement_vs_diversity.pdf}
    \caption{Analyzing the gains of our \NNC{} ensembling method against the diversity in correct predictions across CLIP backbones in the 21 selected benchmarks.}
    \label{fig:imp_div}
\end{figure}

==> sections/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our claims are made through experimental results and comprehensive analysis in 21 datasets. We carefully considered our findings and present multiple results to showcase the importance of them. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We approach the limitations of our method in the section 6. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Through the paper and in specific on the section A in the supplemental material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Through the experiments and in the supplemental material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Throughout the paper we use absolute improvement and the average, maximum and minimum of the gains obtained by the combination of multiple backbones.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Explained in supplemental material section A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have read the NeurIPS Code of Ethics, and our work conforms, in every respect, with the Code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We think that this work present %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't think that our model have a high risk for misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite and reference the code provided by openAI
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't perform research with human subjects or crowdsourcing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> sections/trash-experiments.tex <==
% \input{tables/zs_baselines}
% \input{tables/lp_table}
% \input{tables/lp_baselines}
% \section{Experimental Setup}
% \label{sec:setup}


%Our goal is to assess the performance differences among multiple CLIP backbones in image classification and to improve performance by combining these backbones. We evaluate each backbone's performance and the fusion mechanism using accuracy.
% Our objectives are to evaluate 
% the differences in the multiple backbones used to train CLIP in image classification performance and 
% combine these backbones to enhance the performance in the image classification task. We, therefore, utilize accuracy to evaluate the performance of each backbone of CLIP and the fusion mechanism.

%\textbf{Non-parametric} ensembling baselines include two options.


 %Additionally, we experiment with top-3 voting (\VoteThree), where we seek a consensus among backbones by considering the three most likely predictions from each of them. These predictions are weighted based on their position within the top-3 list.
% \paragraph{\textbf{Confidence} (\Confidence)} Using the Shannon entropy to evaluate the confidence of each backbone in each prediction, we select the backbone with the highest confidence for a prediction as the source of the final prediction.

In this context, we add to the classical ensembling techniques a



% Finally, We evaluate our proposed method against several existing approaches: Tip-Adapter and Tip-Adapter-F~\cite{zhang2021tip}, Zero-Shot CLIP~\cite{radford2021learning}, Linear-probe CLIP~\cite{radford2021learning}, CoOP~\cite{zhou2022learning}, and CLIP-Adapter~\cite{gao2021clip}. Linear-probe CLIP fine-tunes an additional linear classifier on a few-shot training set after freezing the original CLIP. CoOP aims to make prompts learnable by generating different prompt designs. CLIP-Adapter enhances few-shot classification performance by introducing a feature adapter \cite{houlsby2019parameter} on CLIP's visual and textual encoders. This adapter helps to reduce the domain gap between pre-trained and transferred features.
% Tip-Adapter, a training-free variant of CLIP-Adapter, achieves comparable or superior performance without requiring backpropagation for adapter training. Instead, it constructs adapter weights using a key-value cache model from the few-shot training set. Fine-tuning Tip-Adapter can further enhance performance with rapid convergence. All these methods adopt a prompt ensembling of 7 templates for zero-shot.
    % \CRO{Few-shot CLIP Adapter}
% \input{tables/results_table1}
% \input{plots/nnc_zeroshot_clip_barchart}
% \input{plots/nnc_zeroshot_delta}
% \input{plots/nnc_zeroshot_normalized_delta}




%We evaluate our model's performance by combining the zero-shot CLIP backbones. 
% Then, we evaluate the combination of adapted CLIP backbones by linear probing. 
%In this setting, we compare our proposed approach against common ensembling techniques grouped into Non-Parametric and Parametric baselines to assess our proposed approach.

%Some baselines and results are discussed in the main paper, while others are detailed in the Appendix~\ref{app:baselines}.

% Our initial investigation primarily revolves around evaluating the model's performance in comparison to the baseline zero-shot CLIP paradigm. However, our study also encompasses experimental investigations into the differences in adapted CLIPs using linear probing and few-shot setting for combining the backbones.
% To help characterize the improvements that can be achieved with our proposed approach, we consider common model ensembling techniques as baselines, namely logit averaging (\LogitAvg) and voting. Voting enables us to combine conceptually different classifiers and use a majority vote or the average predicted probabilities (soft vote) to predict the class label. For this study, we experiment with two settings. Firstly, we use the top-1 (\VoteOne) prediction from each backbone, and the final prediction is determined by the label with the highest number of votes. In cases where multiple labels receive the same number of votes, we select the one with the highest probability. Additionally, we experiment with top-3 voting (\VoteThree), where we seek a consensus among backbones by considering the three most likely predictions from each of them. These predictions are weighted based on their position within the top-3 list.
% To assess the potential improvements of our proposed approach, we compare it against common model ensembling techniques grouped into Non-Parametric and Parametric baselines. Some of these baselines and results are discussed in the main paper, while others are detailed in the appendix \ref{app:baselines}.




% \input{tables/zs_table}
% \input{tables/lp_results}
% \input{tables/fewshot_nnc}






% \input{tables/tip_adapter_w_nnc_eurosat_fgvc}
% \input{tables/tip_adapter_w_nnc_pets_dtd}
%  We evaluate our proposed method against several existing approaches: Tip-Adapter and Tip-Adapter-F~\cite{zhang2021tip}, Zero-Shot CLIP~\cite{radford2021learning}, Linear-probe CLIP~\cite{radford2021learning}, CoOP~\cite{zhou2022learning}, and CLIP-Adapter~\cite{gao2021clip}. Zero-Shot CLIP performs classification solely based on similarities without using any additional training samples. Linear-probe CLIP fine-tunes an additional linear classifier on a few-shot training set after freezing the original CLIP. CoOP aims to make prompts learnable by generating different prompt designs. We choose its most effective variant for comparison, which includes placing the class token at the end of 16-token prompts and sharing the context across all classes. CLIP-Adapter enhances few-shot classification performance by introducing a feature adapter \cite{houlsby2019parameter} on CLIP's visual and textual encoders. This adapter helps to reduce the domain gap between pre-trained and transferred features.
% Tip-Adapter, a training-free variant of CLIP-Adapter, achieves comparable or superior performance without requiring backpropagation for adapter training. Instead, it constructs adapter weights using a key-value cache model from the few-shot training set. Fine-tuning Tip-Adapter can further enhance performance with rapid convergence. All these methods adopt prompt ensembling of 7 templates for zero-shot.



% \CRO{TODO}
% Analysis! %TODO

% \subsection{Resiliency to augmentations}
% \subsection{Qualitative analysis}

% \input{tables/variability_per_dataset}
% \input{tables/zs_delta_accuracy_per_dataset}
% \input{tables/zs_delta_accuracy_per_augmentations}
% \subsection{Action recognition?}
% \subsection{Name-to-keypoint Keypoint-to-name?}
% \subsection{Video Grounding}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \input{figures/analysis_rnd_proj}
% \todowriting[inline]{Introduce setting}
% \todowriting[inline]{Introduce tasks and datasets}
% \todonum[inline]{Image Classification}
% Try multiple downstream tasks that could take advantage of the alignment of multiple backbones.


% \todonum[inline]{Image retrieval}
% \begin{enumerate}
%     \item MSCOCO
%     \item Flickr30k
% \end{enumerate}
% \todonum[inline]{Action Recognition}
% \begin{enumerate}
%     \item UCF101
%     \item K700
%     \item \st{RareACt}
% \end{enumerate}
% \todonum[inline]{OCR}
% \begin{enumerate}
%     \item MNIST
%     \item SVHN
%     \item IIT5k
%     \item HatefulMemes
%     \item SST-2
% \end{enumerate}
% \todonum[inline]{Geolocalization}
% \begin{enumerate}
%     \item IMG2GPS
% \end{enumerate}
% \todonum[inline]{Robustness to Distribution Shift}
% \begin{enumerate}
%     \item ImageNet
%     \item ImageNet-V2
%     \item ImageNet-A    
%     \item ImageNet-R
%     \item ObjNet    
%     \item ImageNet-Sketch
%     \item ImageNet-Vid    
%     \item \st{YouTube-BB}
% \end{enumerate}


%enables us to combine conceptually different classifiers to predict the class label. It consists of using the majority of votes between the backbones to produce a final prediction. We use the top-1 (\VoteOne) prediction from each backbone, and the final prediction is determined by the label with the highest number of votes. In cases where multiple labels receive the same number of votes, we select the one with the highest probability.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Version with Damien comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Experiments}
% \label{sec:experiments}

% \paragraph{Backbones.}
% We consider the original selection of backbones described by \citet{radford2021learning}.
% This includes the ResNets~\cite{He_2016_CVPR} RN50, RN50x4, RN50x16, RN50x64 and RN101, and the ViTs~\cite{dosovitskiy2020vit} B-16, B-32, L-14 and L-14-336.
% All models are obtained through the open-source project OpenCLIP~\cite{ilharco_gabriel_2021_5143773}.

% \paragraph{Datasets.}
% \label{subsec:db_bkbones}
% We use a selection of 21 popular image classification datasets: \Caltech101{} \cite{li_andreeto_ranzato_perona_2022}, \Cars{} \cite{krause2013collecting}, \Cifarten{} \cite{krizhevsky2009learning}, \Cifaronehundred{} \cite{krizhevsky2009learning}, \Clevr{} \cite{johnson2017clevr}, \Cub{} \cite{WahCUB_200_2011}, \Dtd{} \cite{cimpoi14describing}, \Eurosat{} \cite{helber2018introducing}, \FGVC{} \cite{maji13fine-grained}, \Flowers{} \cite{nilsback2008automated}, \Food{} \cite{bossard2014food}, \Gtsrb{} \cite{Houben-IJCNN-2013}, \Imagenet{} \cite{deng2009imagenet} \Mnist{} \cite{deng2012mnist}, \Pcam{} \cite{Veeling2018-qh}, \Pets{} \cite{parkhi2012cats}, Rendered\Renderedsst2 \cite{socher-etal-2013-recursive}, \Resisc45 \cite{Cheng_2017}, \STL10 \cite{coates2011analysis} and \SUN397 \cite{Xiao:2010}.
% They include diverse images of nature, animals, places, medical scans, satellite images, and man-made objects.
% The evaluation metric is simply the accuracy on the test split of each dataset. The aggregated performance is the average accuracy across all datasets weighted equally.

% \paragraph{Baselines.}
% Our experiments consider several ensembling baselines. Non-parametric approaches:
% \begin{itemize}[topsep=-2pt,itemsep=1pt,labelindent=2pt,labelsep=*,leftmargin=12pt]
% \item \textbf{Logit averaging} (\LogitAvg) simply takes the average of the logits (scores) of the models.

% \item \textbf{Voting} (\VoteOne{})
% uses a majority vote. Each model casts a vote for its max-scored class.
% The final prediction is the class with the highest number of votes.
% Compared to \LogitAvg, this does not use the \emph{soft} score values and the uncertainty reflected therein.
% \end{itemize}
% Parametric approaches:
% \begin{itemize}[topsep=-2pt,itemsep=1pt,labelindent=2pt,labelsep=*,leftmargin=12pt]
% \item \textbf{Calibrated logit averaging} (\CLogitAvg)
% first calibrates each model independently using temperature scaling.
% They are then combined by simply averaging their logits.
% \item \textbf{Genetic Algorithm} (\GAC) \CRO{explain this and why we want to do it}
% \item \textbf{Mixtures of experts (MoE)} are a popular method to improve performance by combining specialized submodels~\cite{NEURIPS2022_91edff07, lepikhin2020gshard, rau2019moe, Zoph2022STMoEDS}.
% MoEs split a model into experts that each focus on a specific input region. A gating network determines which expert is relevant for a given input.
% %, coordinating their collaboration.
% We use the Sparse MoE implementation~\cite{Zoph2022STMoEDS} by \citet{rau2019moe}, where the MoE layer's input is the concatenation of vision features $x_b$ from $\phi_b$. We use standard hyperparameters: $9$ experts trained for classification with cross-entropy loss with Adam \cite{kingma2014adam} and a learning rate of $2\mathrm{e}{-5}$ for 300 epochs.
% \end{itemize}\vspace{1pt}

% See Appendix~\ref{app:baselines} a discussion of additional baselines.
% The appendix also contains additional results on
% the combination of backbones and how they perform
% under distribution shifts on the \Imagenet{} dataset (Section~\ref{app:robustness}). We also present additional evaluation of the computational efficiency using the Cascade framework~\cite{wang2022wisdom} in (Section~\ref{app:efficiency}).
% Finally, Section~\ref{app:alpha_values} presents
% dataset-specific results including
% overlap diagrams, an analysis of possible model combinations using \NNC{} and our \Oracle{}, as well as the dataset-specific learned temperature values. 

% \subsection{Combination of Backbones}
% % \DT{FIRST, OUTLINE THE EXPERIMENTS AND WHAT YOU SEEK TO SHOW/DEMONSTRATE.}

% % The challenges of effectively fusing different backbones for improved predictions are evident in Figure~\ref{fig:barchar_nnc_zs} (Table~\ref{tab:zs-baselines}). Our experiments aim to compare non-parametric and parametric methods for combining multiple backbones to enhance prediction accuracy. Specifically, we seek to demonstrate the limitations of simple averaging approaches and the efficacy of our proposed method, \NNC{}, in leveraging the strengths of diverse backbones.
% In this experiment, we compare non-parametric and parametric techniques for merging multiple CLIP backbones that are not adapted for each specific task. We aim to show the limitations of averaging methods and the superior performance of our \NNC{} approach, which effectively utilizes the strengths of various backbones. Figure~\ref{fig:barchar_nnc_zs} (Table~\ref{tab:zs-baselines}) highlights the performance of each fusion techniques.
% In non-parametric baselines, 
% using the \LogitAvg{} approach consistently fails to enhance the overall performance beyond that of the best backbone. Thus, averaging performance across backbones does not exploit their complementarity between predictions effectively, yielding an average delta accuracy of 1.3\%. Notably, the \LogitAvg{} approach shows substantial improvement for the \Country{} dataset compared to the best backbone. When the backbones are calibrated \CLogitAvg{}, the \LogitAvg{} approach enhances its performances across all datasets except \Gtsrb{}, \Mnist{}, \Resisc45{}, and \SUN397{} when compared to the non-calibrated version. Intriguingly, \textbf{Vote T-1} proves ineffective in significantly boosting prediction accuracy beyond that of the best backbone.
% In employing parametric methods, we utilize the entire training set of the target datasets. Our proposed approach \NNC{} demonstrates a noteworthy capability to enhance the performance of the best backbone, achieving a substantial improvement of up to 35.1\% in the case of the \Eurosat{} dataset. On average, our method exhibits a commendable improvement of 8.1\% compared to the \Best{} backbone's performance across the evaluated datasets.

% % leveraging the confidence of each backbone in its predictions consistently fails to enhance the overall performance beyond that of the best backbone. 
% % The lack of calibrated probabilities in the \Confidence{} contributes to overconfidence in some backbones, resulting in performance degradation when combined.
% % Calibrating the confidence leads to improvements, although the performance still falls short of matching the best backbone, except for \Dtd{}, \Caltech101{}, \Eurosat{} and \Cars{}. 
% % This trend persists in the \LogitAvg{} approach, where averaging performance across backbones does not exploit their complementarity between prediction effectively, yielding an average delta accuracy of 0.1\%. Notably, the \LogitAvg{} approach shows substantial improvement for the \Cub{} dataset compared to the best backbone. When the backbones are calibrated \CLogitAvg, the \LogitAvg{} approach enhances its performances across all datasets except \Gtsrb, \Mnist, \Resisc45, and \SUN397 when compared to the non-calibrated version. Intriguingly, conventional ensemble techniques such as \textbf{Vote T-1} and \textbf{Vote T-3} prove ineffective in providing a significant boost to prediction accuracy beyond that of the best backbone.
% % In the parametric methods, we use the total train set of the target datasets. Our proposed approach is capable to improve the performance of the best backbone up to 6.34\% in the case of \CUB{} dataset. In average, it presents an improvement of 2.69\% when we compare our method with the performance of the Best backbone.
% % As we can see in Table \ref{tab:zs-baselines}, fusing the different backbones' to improve the predictions is not simple. In the non-parametric baselines, it is consistent that using the confidence of a backbone in its predictions does not help to improve the performance of the best backbone. Since the probabilities are not calibrated in this case, some backbones are expected to be overconfident in their predictions, making the performance drop when we want to combine them. However, as we can see in the calibrated confidence, the performance improves by independently calibrating each backbone's probabilities. Still, it cannot reach the best backbone's performance except for \DTD. 
% % The same behaviour can be seen in the logit averaging approach. Overall, averaging the performance does not correctly combine the backbones to use their orthogonal prediction power, obtaining an average delta accuracy of -0.85\%.  This approach can significantly boost the \CUB{} dataset when we compare it with the best backbone. After calibrating the probabilities of each backbone, the logit averaging approach improves its performance across all datasets but \CUB, \Food and \Imagenet{}, when we compare with the logit averaging without calibration. 
% % Interestingly, the standard approaches used on ensembles like Voting are far from helping to get a boost that improves the best backbone's prediction accuracy.  

% % Using the zero-shot predictions, we evaluate its ``orthogonality'' in the predictions by two experiments. First, we create an oracle prediction that know what backbone to use for each image sample in the dataset. Although the combination of probabilities could bring even better performance, we consider this as a reasonable upperbound to evaluate the potential in combining this backbones. As seen in Table~\ref{tab:zs-table}, the upperbound is always better than the best backbone. Remarkably, FGVC\_Aircraft, CUB and Cars obtained an improvement of 20.38\%\, xx and xx. Secondly, we plot the Venn diagram of the predictions and visually inspect what are the differences and commonalities in the predictions, we present the results in ImageNet in Figure \ref{fig:venn_diagram}, for the other datasets please see the Appendix.

% \subsection{Linear Probes}
% \DT{MOTIVATION + DESCRIPTION OF EXPERIMENTS OF THIS SECTION.}
% We also investigate each backbone's adaptability and \textit{complementarity} when subjected to adaptation for a specific dataset. This examination aims to understand how effectively each backbone can be tailored to a target dataset's characteristics and determine if \textit{complementarity} remains after adaptation.
% This adaptation is facilitated through the use of \textbf{linear probing}, which is a more straightforward and effective methodology compared to comprehensive fine-tuning of pre-trained models. Linear probing employs a frozen pre-trained backbone with a linear layer for efficient learning of a dataset-specific classifier.
% % This adaptation is facilitated through the utilization of \textbf{linear probing}. 
% % In contrast to a comprehensive fine-tuning of the pre-trained models, linear probing emerges as a more straightforward and effective methodology for tailoring foundational models to a target dataset. 
% % The linear probing technique employs a linear layer, wherein the weights of the pre-trained backbone remain frozen, allowing for the efficient learning of a classifier tailored to the attributes of the specific dataset.
% We initialize the weights of the linear probing using language weights, as detailed in~\cite{li2022elevater}. This initialization strategy is notably superior to random initialization, showing enhanced stability, especially in few-shot learning scenarios.
% % We initialize the weights of the linear probing using language weights, a practice detailed in~\cite{li2022elevater}. This initialization strategy proves notably superior to random initialization, exhibiting enhanced stability, particularly in scenarios involving few-shot learning. 
% We use the output of each backbone $\phi_b$ normalized with L2 as input to the linear probing. Each linear probe is trained using 90\% of the target dataset's training set, reserving the remaining 10\% for integrating the backbones using \NNC{}.
% % We use the output of each backbone $\phi_b$ normalized with L2 as an input to the linear probing. Each linear probe undergoes training with the target dataset's training set, allocating 90\% for the actual linear probe training and reserving the remaining 10\% for \NNC.


% \input{plots/nnc_zeroshot_clip_barchart}
% \input{plots/nnc_linearprobe_clip_barchart}
% \begin{wraptable}[10]{RH}[0pt]{0.45\textwidth}
% \caption{Classification accuracy of models under few-shot settings.}
% \label{tab:comparison}
% \centering      
% \resizebox{0.45\textwidth}{!}{
%         \begin{tabular}{lccccc}
%         \toprule
%          Few-shot  & 1 & 2 & 4 & 8 & 16 \\
%          \midrule
%         Linear-probe CLIP \cite{radford2021learning} & 22.2 & 31.9 & 41.2 & 49.5 & 56.1 \\
%         CoOP\cite{zhou2022learning} & 47.6 & 50.9 & 56.2 & 59.9 & 63.0 \\
%         CLIP-Adapter\cite{gao2021clip} & 61.2 & 61.5 & 61.8 & 62.7 & 63.6 \\
%         Tip-Adapter\cite{zhang2021tip} & 60.7 & 61.0 & 61.0 & 61.5 & 62.0 \\
%         Tip-Adapter-F\cite{zhang2021tip} & 61.3 & 61.7 & 62.5 & 64.0 & 65.5 \\
%         \midrule
%         \NNC & \textbf{78.2} & \textbf{78.1} & \textbf{78.2} & \textbf{78.3} & \textbf{78.4} \\
%          \bottomrule
%         \end{tabular}%
% }
% \end{wraptable}
% Figure \ref{fig:nnc_lp} (Table~\ref{tab:lp-baseline}) presents results from combining linear probing versions for each backbone, using both non-parametric and parametric approaches. Similar to the zero-shot setting, our proposed \NNC{} consistently improves performance across all datasets, with an average enhancement of 1.6\% compared to the \Best{} linear-probe backbone. This improvement is less evident than the combination of the zero-shot version. Interestingly, the \textbf{MoE} approach does not reach the performance level of the best backbone in several benchmarks and shows a maximum degradation of -20.9\%. This suggests that MoE may struggle to partition the input space effectively into distinct clusters, specific to certain experts, potentially limiting its functionality.

% % Figure \ref{fig:nnc_lp} (Table~\ref{tab:lp-baseline}) showcases the results of combining linear probing versions for each backbone, using both non-parametric and parametric approaches. Similar to the zero-shot setting, our proposed \NNC{} consistently demonstrates improvement across all datasets, achieving an average enhancement of 1.6\% compared to the \Best{} linear-probe backbone. Notably, this improvement is more modest than the combination of the zero-shot version, which records an average improvement of 8.1\%. Intriguingly, the MoE approach does not reach the performance level of the \Best{} backbone in multiple benchmarks and exhibits a maximum degradation of -20.9\%. This discrepancy suggests that MoE might face challenges in effectively partitioning the input space into distinct clusters specific to certain experts, potentially hindering its optimal functionality.
% %Notably, a substantial enhancement in performance is observed through this adaptation technique when compared to the zero-shot \LTwo Norm (Table~\ref{tab:zs-all-table}).
% % RN50 stands out as the backbone experiencing the most significant improvement, averaging a remarkable 23.5\% across all datasets, surpassing even ViT-B-32. Despite this, its performance falls short of outperforming other backbones. Even after linear probing, ViT-L-14 and ViT-L-14-336 remain the top-performing backbone across all datasets. Noteworthy is the considerable room for improvement indicated by the \Oracle{} of linear probes, showcasing superior performance compared to any individual backbone, suggesting potential gains through a combination of backbones. 
% % Although the room for improvement between the \Oracle{} and the best linear probe is consistent across datasets, we found that the space for improvement is less than the zero-shot option. %In overall \CRO{Continue}

% % \CRO{Combination of backbones}
% % \CRO{setup}
% % \input{tables/fewshot_nnc}
% % \input{tables/lp_only_fewshot}
% % We can see in Table \ref{tab:lp-baselines} the results of combining the linear probing of each backbone using the baselines and our proposed approaches. Similar to the results in the zero-shot setting, our proposed \NNC{} obtained a consistent improvement across all datasets, with an average improvement of 0.85\% with respect to the \Best{} linear-probe backbone. The improvement is much less than the zero-shot version, which record an average improvement of 2.69\%. 
% % Interestingly, the MoE is not reaching the performance of the \Best{} backbone and obtains a negative improvement of -3.68\%. It is very likely that MoE are not working properly since it is not capable to divide the input space in notorious clusters that are later specific task for certain expert. 

% \subsection{Comparison with Few-Shot Adapter Methods}
% % \input{tables/tip_adapter_comparison}{\parfillskip=0pt\par}
% \DT{MOTIVATION OF THESE EXPERIMENTS.}
% We now compare our method against Tip-Adapter, Tip-Adapter-F~\cite{zhang2021tip}, few-shot Linear-probe CLIP~\cite{radford2021learning}, CoOP~\cite{zhou2022learning}, and CLIP-Adapter~\cite{gao2021clip}. Linear-probe CLIP fine-tunes a linear classifier on a few-shot training set on the frozen CLIP backbones. CoOP~\cite{zhou2022learning} generates different prompt designs to make prompts learnable. CLIP-Adapter~\cite{gao2021clip} enhances few-shot classification by introducing a feature adapter on CLIP's visual and textual encoders. Tip-Adapter~\cite{zhang2021tip} achieves comparable performance to CLIP-Adapter without requiring training, using a key-value cache model from the few-shot training set. Tip-Adapter-F can further enhance performance by fine-tuning the cache. %All methods use a prompt ensemble of 7 templates for zero-shot.
% As shown in Table \ref{tab:comparison}, our \NNC{} shows an outstanding performance over compared methods and consistently surpasses other few-shot methods by learning how to combine multiple backbones, which is a complementary approach to any of these adapters. In Supplemental Material, Table \ref{tab:few_shot_bbone}, we show that current few-shot adapter methods also have performance differences with various backbones, and still, our \NNC{} surpassed the best backbone reported by their method. 

% \input{plots/tipadapter_nnc}
% \begin{wrapfigure}[17]{RH}[0pt]{0.4\textwidth}
%     \includegraphics[width=0.4\textwidth]{figures/clevr_alphas.pdf}
%     \caption{Distribution of the temperature values learned, normalized by their maximum value, by our \NNC{} method on the \Clevr{} dataset}
%     \label{fig:alpha_box_plots_eurosat_mainpaper}
%     % \hfill
% \end{wrapfigure}
% Moreover, we integrate Tip-Adapter~\cite{zhang2021tip} with our \NNC{} ensembling mechanism and conduct experiments on \Eurosat{}, \FGVC{}, \Dtd{}, and \Pets{}. Initially, we apply Tip-Adapter and Tip-Adapter-F independently on each backbone, following their protocol with 1, 2, 4, 8, and 16 shots. Subsequently, we employ our ensembling mechanism to fuse the adapted backbones. For training \NNC{}, we utilize the validation set used by Tip-Adapter to linearly combine their logits with CLIP.



% See Figure~\ref{fig:tipadapter_nnc} (Tables \ref{tab:eurosat_tannc}--\ref{tab:pets_tannc}) for a comparison of the performance of Tip-Adapter over different zero-shot CLIP backbones, and the combination of all these Tip-Adapter versions with \NNC. Across the four datasets used in these experiments, \NNC{} improves over each version of Tip-Adapter in the few-shot setting. Notably, \NNC{} for \Eurosat{} shows an improvement of up to 10\% with respect to the best Tip-Adapter backbone (L-14-336) using 16 shots.

% \subsection{Examining the Learned Temperature Values}
% We visualise the learned temperature values to understand how the \NNC{} method assigns weights to different backbones and reveal its strategy for leveraging the strengths of diverse architectures to enhance prediction accuracy. 
% Figure \ref{fig:alpha_box_plots_eurosat_mainpaper} shows the learned temperature values for \NNC{} on the \Clevr{} dataset, other datasets in Section \ref{app:alpha_values}.
% By examining the learned temperature values, the experiment assesses the contribution of each backbone, 
% noting that the most weighted backbone is not consistently the deepest one, such as ResNet-101. 
% The uniform distribution of learned temperatures across backbones indicates that \NNC{} effectively utilizes the strengths of multiple backbones, resulting in a more balanced and accurate labeling process, complementing our analysis in Figure \ref{wrap-fig:improvement_vs_diversity}.
% These findings highlight that \NNC{} benefits from the diversity in model predictions, reinforcing the advantage of combining various backbones.

% % Notably, there is a slight dominance in the temperature values for the ResNet family of backbones. However, it is observed that the most weighted backbone within the ResNet family is not consistently ResNet-101, despite its deeper architecture. Furthermore, the distribution of weights across backbones for datasets is very uniform. This suggests that the \NNC{} method is effectively leveraging the strengths of each backbone to arrive at accurate labels for each sample, resulting in a more balanced distribution of weights across different backbones, complementing our analysis in Figure \ref{wrap-fig:improvement_vs_diversity}

--


% leveraging the confidence of each backbone in its predictions consistently fails to enhance the overall performance beyond that of the best backbone. 
% The lack of calibrated probabilities in the \Confidence{} contributes to overconfidence in some backbones, resulting in performance degradation when combined.
% Calibrating the confidence leads to improvements, although the performance still falls short of matching the best backbone, except for \Dtd{}, \Caltech101{}, \Eurosat{} and \Cars{}. 
% This trend persists in the \LogitAvg{} approach, where averaging performance across backbones does not exploit their complementarity between prediction effectively, yielding an average delta accuracy of 0.1\%. Notably, the \LogitAvg{} approach shows substantial improvement for the \Cub{} dataset compared to the best backbone. When the backbones are calibrated \CLogitAvg, the \LogitAvg{} approach enhances its performances across all datasets except \Gtsrb, \Mnist, \Resisc45, and \SUN397 when compared to the non-calibrated version. Intriguingly, conventional ensemble techniques such as \textbf{Vote T-1} and \textbf{Vote T-3} prove ineffective in providing a significant boost to prediction accuracy beyond that of the best backbone.
% In the parametric methods, we use the total train set of the target datasets. Our proposed approach is capable to improve the performance of the best backbone up to 6.34\% in the case of \CUB{} dataset. In average, it presents an improvement of 2.69\% when we compare our method with the performance of the Best backbone.
% As we can see in Table \ref{tab:zs-baselines}, fusing the different backbones' to improve the predictions is not simple. In the non-parametric baselines, it is consistent that using the confidence of a backbone in its predictions does not help to improve the performance of the best backbone. Since the probabilities are not calibrated in this case, some backbones are expected to be overconfident in their predictions, making the performance drop when we want to combine them. However, as we can see in the calibrated confidence, the performance improves by independently calibrating each backbone's probabilities. Still, it cannot reach the best backbone's performance except for \DTD. 
% The same behaviour can be seen in the logit averaging approach. Overall, averaging the performance does not correctly combine the backbones to use their orthogonal prediction power, obtaining an average delta accuracy of -0.85\%.  This approach can significantly boost the \CUB{} dataset when we compare it with the best backbone. After calibrating the probabilities of each backbone, the logit averaging approach improves its performance across all datasets but \CUB, \Food and \Imagenet{}, when we compare with the logit averaging without calibration. 
% Interestingly, the standard approaches used on ensembles like Voting are far from helping to get a boost that improves the best backbone's prediction accuracy.  

% Using the zero-shot predictions, we evaluate its ``orthogonality'' in the predictions by two experiments. First, we create an oracle prediction that know what backbone to use for each image sample in the dataset. Although the combination of probabilities could bring even better performance, we consider this as a reasonable upperbound to evaluate the potential in combining this backbones. As seen in Table~\ref{tab:zs-table}, the upperbound is always better than the best backbone. Remarkably, FGVC\_Aircraft, CUB and Cars obtained an improvement of 20.38\%\, xx and xx. Secondly, we plot the Venn diagram of the predictions and visually inspect what are the differences and commonalities in the predictions, we present the results in ImageNet in Figure \ref{fig:venn_diagram}, for the other datasets please see the Appendix.


% We also investigate each backbone's adaptability and \textit{complementarity} when subjected to adaptation for a specific dataset. This examination aims to understand how effectively each backbone can be tailored to a target dataset's characteristics and determine if \textit{complementarity} remains after adaptation.
%Motivation



%potential to dataset-specific adaptability and \textit{complementarity} when subjected to adaptation for a specific dataset. We aim to understand how effectively each backbone can be tailored to a target dataset and determine if \textit{complementarity} remains after adaptation. We employ linear probing, a straightforward and effective methodology that uses a frozen pre-trained backbone with a linear layer for efficient learning of a dataset-specific classifier. This setup allows us to evaluate the performance and interplay of each backbone in different contexts.

% In this experiment, we aim to investigate each backbone's adaptability and \textit{complementarity} when subjected to adaptation for a specific dataset. We aim to understand how effectively each backbone can be tailored to a target dataset's characteristics and determine if \textit{complementarity} remains after adaptation. This will provide insights into the robustness and flexibility of different backbones under specific conditions.

%Description
%This examination is facilitated through the use of \textbf{linear probing}, a straightforward and effective methodology compared to comprehensive fine-tuning of pre-trained models. Linear probing employs a frozen pre-trained backbone with a linear layer for efficient learning of a dataset-specific classifier.


% This adaptation is facilitated through the use of \textbf{linear probing}, which is a more straightforward and effective methodology compared to comprehensive fine-tuning of pre-trained models. Linear probing employs a frozen pre-trained backbone with a linear layer for efficient learning of a dataset-specific classifier.
% We initialize the weights of the linear probing using language weights, as detailed in~\cite{li2022elevater}. This initialization strategy is notably superior to random initialization, showing enhanced stability, especially in few-shot learning scenarios.


==> sections/trash.tex <==
% Large pre-trained models, also known as Foundation Models (FMs), are reshaping the landscape of learning, particularly in computer vision \cite{radford2021learning, he2022masked, kirillov2023segment, liu2023improved} and natural language processing \cite{devlin2018bert,brown2020language,Touvron2023LLaMAOA}. 
% These models are trained through self-supervised and contrastive learning objectives on internet-scale data, eliminating the need for manual annotations \cite{jia2021scaling,schuhmann2022laion}. 
% Contrastive Language Image Pre-training (CLIP)~\cite{radford2021learning} stands as a pioneering contribution in the ongoing research endeavours within this domain, establishing itself as the state-of-the-art across diverse downstream tasks. The training objective is to align text and image representations. This versatile framework is applicable to a wide range of commonly used architectures, facilitating the training of general image representation learning models.
% Post-training, quantifying similarities between text and images is facilitated by a straightforward dot product operation applied to their corresponding representations. 

% These representation learning models have significantly advanced the field by serving as the foundational framework for other applications, producing state-of-the-art performance in various cross-modal alignment tasks, including but not limited to zero-shot classification \cite{Zhai_2022_CVPR,li2022elevater,jia2021scaling}, cross-modal retrieval \cite{li2020unicoder,li2020oscar,yu2022coca}, and the evaluation of machine-generated captions \cite{lee2020vilbertscore,jiang2019tiger}.


%can be used to train various 's versatility extends to different architectures, enabling the training of general image representation models. 
%Post-training, similarity quantification between text and images is simplified through a dot product operation on their representations. These models have significantly advanced the field by serving as the foundational framework for other applications, producing state-of-the-art performance 
%in various cross-modal alignment tasks such as


%%%%%%%%%%%%%%%%%%%
% Despite the extensive body of prior research on CLIP, there remains a notable gap when it comes to examining the image representations from the different backbones used to train with CLIP. While we find extensive work evaluating the backbones employed across various tasks to showcase the generalization capabilities of specific methods \cite{goldblum2023battle, li2022elevater, zhang2021tip, gao2021clip}, they typically exhibit general performance improvements when using larger models. This supports the prevailing perception that larger models inherently lead to better representations, implying that they not only learn the same patterns but also more. If true, increasing the model's size alone is enough to improve generalization. However, even within the same family of backbones, architectural selections exhibit nuanced inductive biases, capturing distinct patterns by different representations~\cite{inductive_bias}. Nevertheless, there is a conspicuous absence in thoroughly examining the synergies and variances among these backbones as learned by CLIP, particularly considering their shared training dataset and learning objective.

% To address this gap, we conduct an empirical study to explore the complexities of backbones in the CLIP framework. Our evaluations uncover significant differences in the behaviour of these backbones. They effectively recognize various patterns in the input, leading to different predictions. Furthermore, they demonstrate a distinctive resilience to input image variations and underscore potential synergies between different backbones.

%suggesting that scale alone might be a solution to better generalization.
%, supporting the idea that larger models learn more patterns and suggesting that increasing the model's size alone improves generalization.
%However, architectural choices other than scale also influence the learned representations.

%We discover significant differences.
%and potential synergies across backbones.
%compensate for one another's shortcomings.


%%%%%%%%%%%%%%%%%%%
% This distinctive behaviour suggests that when combined, these backbones can compensate for each other's shortcomings. This complementarity could allow CLIP to maintain robust performance across a wide range of image variations and enhance its overall effectiveness in various applications.

%various applications.
%%%%%%%%%%%%%%%%%%%


% Based on these findings, we propose an ensemble strategy that adaptively integrates diverse backbones within the CLIP framework. 
% Although traditional ensembling techniques, which typically involve averaging the outputs from each backbone, might appear straightforward, our findings indicate that these methods fall short of delivering the desired boost in performance.
% Instead, our method learn an specific temperature scaling to weigh the contribution of each backbone, leading to a final prediction.

%%%%%%%%%%%%%%%%%%%%%%

% To determine these temperatures, we explore two approaches: (1) utilizing a genetic algorithm as a search strategy and identifying a dataset-specific value, and (2) employing a multi-layer perceptron (MLP) to learn and adjust these temperatures individually for each sample. We observe that MLP efficiently learns to predict these temperatures with very few samples. We call this approach neural network combinator (NNC).
% This method allows for the seamless integration of information from different backbones, contributing to improved predictive performance. 
% \CRO{Here, talk about Figure 2.} 
% Our method surpasses strong state-of-the-art CLIP adapter methods~\cite{zhang2021tip,gao2021clip,zhou2022learning,radford2021learning}. It also outperforms the state-of-the-art few-shot learning method~\cite{zhang2021tip}. Notably, our approach is both orthogonal and complementary to these existing approaches.


%The method is called Neural Logit Controller (\NNC{})

%This improves predictive performance through seamless integration of information from different backbones.

%We found that these baselines (parametric and non-parametric methods)
%, falling short of delivering the desired boost in performance.

%, considering the respective strengths and weaknesses of others, enhances prediction accuracy.



% \damien{Need to explain what the 'modality gap' means or replace with a few words that are more explicit ("separation of image and text embeddings in CLIP's joint latent space") and say why it supports your method. If that's too long for the intro, I would drop mentioning it here.}
%diverse performance outcomes when manipulating the logits in CLIP and backbone-specific modality gap~\cite{clip-understanding}.

--

% We achieve this by computing a compatibility score ($\text{score}(x,l) = \phi_v(x)^\top \phi_l(l)$) between the encoded inputs.
% Based on these principles, to perform zero-shot image classification using CLIP, we follow previous work and generate prompts that encapsulate the labels of the target dataset (e.g., \texttt{an image of \{label\}, which is a \{concept\}}). Subsequently, we calculate the similarity between the image feature $\phi_v(x)$ and the prompt representations $\phi_l(y)$, where $y$ represents a label within the class set. The prompt exhibiting the highest similarity is then chosen as the label for the given image. 
% and the joint probability distribution that is proportional to the exponentiated dot product of their representations, as shown in Equation (\ref{equation:score_prob}). 
% \begin{equation}
%     \text{score}(x,l) = \phi_v(x)^\top \phi_l(l),
%     \qquad
%     p(x,l) \propto \exp\big(\phi_v(x)^\top \phi_l(l)\big)  
%     \label{equation:score_prob}
% \end{equation}
% For a downstream classification task with label set \sY, we can compute the conditional probability distribution over labels as:
% ppre(\by∣\bx)=exp(⟨\phiv(\bx),\phit(\by)⟩)∑\by′∈\bYexp(⟨\phiv(\bx),\phit(\by′)⟩)ppre(\by∣\bx)=∑\by′∈\bY​exp(⟨\phiv(\bx),\phit(\by′)⟩)exp(⟨\phiv(\bx),\phit(\by)⟩)
% where labels \by\by are represented in their textual form, leveraging the pre-trained model's capabilities for open-ended tasks. The predicted label is then given by \by⋆=argmax\by′∈\bYppre(\by′∣\bx)\by⋆=argmax\by′∈\bY​ppre​(\by′∣\bx).
% Contrastive Language-Image Pretraining, a framework known as CLIP, is designed to align images and their textual descriptions through a self-supervised learning objective. This alignment is crucial, as it enables us to map textual or visual inputs, processed by their respective neural encoders denoted as $\phi_l$ and $\phi_v$, to a unified semantic space. We achieve this by computing a compatibility score between the encoded inputs, as shown in Equation (\ref{equation:score}).
%One way to use this approach is to consider the joint probability of image $x$ and its corresponding description in natural language $l$ is proportional to a compatibility score between them, which we compute as the inner product between the encoded inputs, as Equation \ref{equation:score} shows below.
% \begin{equation}
%     \text{score}(x,l) = \phi_v(x)^\top \phi_l(l)
%     \label{equation:score}
% \end{equation}
% To construct a probability distribution from these scores, we use the exponential function, thus allowing us to write the relationship shown below.
% In Equation \ref{equation:jointprobs}, $x$ and $l$ denote the visual and language inputs that live in spaces $\sX$ and $\sL$ of possible inputs to the model, respectively.  Then, given a downstream multi-class classification task with the label set $\sY \subset \sL$ and $|\sY|=C$, we can write the following.
% Given a downstream multi-class classification task with the label set $\sY \subset \sL$ and $|\sY|=C$,  we can compute the probability distribution over labels as follow
% \begin{align}
%     p(y \mid x) &= \frac{\exp\big(\phi_l(y)^\top \phi_v(x)\big)}{\sum_{y \in \sY} \exp\big(\phi_l(y)^\top \phi_v(x)\big)}\,, 
%     \quad y^\star = \arg\max_{y'\in Y} p(y' \mid x)\,. \label{eq:clip_prediction}
% \end{align} % \label{eq:clip_prediction} 
% Based on these principles, to perform zero-shot image classification using CLIP, we follow previous work and generate prompts that encapsulate the labels of the target dataset (e.g., \texttt{an image of \{label\}, which is a \{concept\}}). Subsequently, we calculate the similarity between the image feature $\phi_v(x)$ and the prompt representations $\phi_l(y)$, where $y$ represents a label within the class set. The prompt exhibiting the highest similarity is then chosen as the label for the given image. 

% %% this is where out "proposals" start, in my opinion
% Since our interest is to combine multiple CLIP backbones operating simultaneously in this fashion, our first key insight is to note that Equation \ref{eq:clip_prediction} is essentially equivalent to computing a softmax over a vector of logit-like values $\bar{\vz} \in \sR^{C}$, whose entries are constructed using on the inner product between a given input $x$ and the set of labels $\sY$. Concretely, let $\bar{\evz}_c$ denote the c-th entry in vector $\bar{\vz}$, then we define the following.
% \begin{equation}
%     \bar{\evz}_c =  \phi_l(y_c)^\top \phi_v(x) \quad \forall c = [1, \ldots, C]
%     \label{equation:logit-like}
% \end{equation}
% We can use the equation above to rewrite Equation \ref{eq:clip_prediction} simply as $p(y|x) = \text{softmax}(\bar{\vz})$, meaning that we can now essentially equate the output of our zero-shot CLIP classification pipeline, to that of a regular classifier, and interpret the output as a probability distribution over the label space $\sC$.

% Since we are interested in combining backbones, we note that a key goal when constructing traditional model ensembles, a technique often used to combine different models, is to increase robustness by increasing the overall confidence of the predictions. In the supervised setting, confidence is generally measured as the probability associated with the predicted label. Though it is expected that a network should provide a calibrated confidence measure in addition to its prediction, it has been shown that deep neural nets are poorly confidence calibrated \cite{guoCalibrationModernNeural2017}. 

--


%Concretely, we propose to assess the difference of zero-shot predictions by means of two approaches. Firstly, we establish an \Oracle{} prediction that is informed about the appropriate backbone to select for each image sample in the target dataset. Secondly, we propose to employ Venn diagrams to visually analyze the discrepancies and overlaps in predictions, which allows us to characterize the nature of the distinctive predictions across models qualitatively.
% Table \ref{tab:zs-all-table} summarizes the results of CLIP in the image classification task. We first see that the performance between backbones with a similar number of parameters from different families can achieve notable differences in performance. For example, ViT-B-32 performs much better than ResNet-50x4 in the \Cifarten{} and \Cifaronehundred{} benchmarks. However, this is inconsistent across all datasets, as seen in \Imagenet{}. Furthermore, it is observed that a greater number of parameters does not always exhibit better performance compared to a lower number of parameters across the different families of backbones.

% Notably, we see that on \Eurosat, \Clevr, \Cub, \Dtd, \Cifaronehundred{} and \Cars{} the oracle with combination of all possible backbones exhibits improvements of 43.5\%, 36.0\%, 25.1\%, 21.8\%, 16.6\% and 16.0\%, respectively. 


and raises the question of how to exploit this to enhance classifier performance.
%This highlights that the \textit{complementarity} between different backbones is evident and opens the question of how to exploit this to enhance the performance of a classifier.

--

%Additionally, there is agreement in predictions within each family of backbones, with just $26,678$ instances correctly predicted by all ViT backbones and $22,358$ shared across all ResNet backbones.
%This suggests that each family

% In qualitative terms, as shown in Figure \ref{fig:venn_diagram} via a Venn diagram with the correct predictions of each backbone on ImageNet-1k \cite{deng2009imagenet}, we see that ViT-L-14-336 and RN50x64 accurately predict 38.285 and 36.963 images from the test set, respectively. Also, we can see the agreement in prediction in each family of backbones, in the ViT family just 26.680 instances are correctly predicted by all the ViT backbones. In the ResNet family, 22.367 are shared across all the backbones in that set. 


% \damien{The "Venn diagram" figure is not intuitive because the order of the columns seems random. Why not use a similar systematic ordering across the 3 diagrams? (e.g. all columns with 1 agreement, followed by all columns with 2 agreements, etc.) Maybe also mention in the caption that there are $(2^\textrm{nModels}\!-\!1)$ columns, this should help the reader check his understanding of what it represented. Another option would be to represent the 3rd as an actual Venn diagram (overlapping circles).}

% Leveraging the informed \Oracle{} using ResNet, ViT, All increases the overall correct predictions to $42426$, $42276$ and $44506$ samples respectively of $50000$. Notably, each backbone exhibits correct predictions that are unique to that specific backbone. In the \Oracle{} applied to the ResNet family, RN50, RN101, RN50x4, RN50x16 and RN50x64 contribute to $566$, $455$, $518$, $782$ and $1745$ exclusive predictions, respectively. In the \Oracle{} applied to the ViT family, B-32, B-16, L-14 and L-14-336 present 903, 904, 543 and 818 unique predictions, respectively. Finally, when we used all the backbones, we can see that each family contribute with exclusive predictions, \ie, ResNet with $2230$ and ViT with $2080$ exclusive predictions. We highlight that predictions within each backbone family do not constitute a subset of the best model's predictions in each family

--

% \begin{wrapfigure}[17]{RH}[0pt]{0pt}%{r}{0.4\textwidth}
%     \centering
%     \begin{adjustbox}{width=0.4\textwidth, keepaspectratio}
%     \input{plots/augmentation_kiviat.tikz}
%     \end{adjustbox}
%     \caption{Impact of artificial alterations of the input image on each backbone in terms of delta accuracy concerning the original performance}
%     \label{wrap-fig:augmentation}
% \end{wrapfigure} 


% Based on these empirical findings, we hypothesize that we can effectively improve the classification performance by learning to combine CLIP backbones. Thus, we propose an approach that is directly inspired by previous work on network calibration, but extended to multiple model combinations. Concretely, our framework can be regarded as a set of variations of Platt scaling \cite{platt1999probabilistic}. In Platt scaling, the logits of a model are used as features for a logistic regression model, which is trained on the validation set to return probabilities. More concretely, given logit scores $z_i$ for an example $i$, Platt scaling learns scalar parameters $a, b \in \sR$ and outputs $\hat q_i = \sigma(a z_i + b)$ as the calibrated probability. Parameters $a$ and $b$ can be optimized using the NLL loss over the validation set, but during this time, the parameter of the original model are fixed. 

% \todonum[inline]{Difference in the prediction between backbones from the same family used to train CLIP}
% \todonum[inline]{Difference in the prediction between families of backbones used to train CLIP}
% \todonum[inline]{Measure the bias of each of the backbone using, paper []}
% \todonum[inline]{Explore the width of the backbone, paper [].}
% \todonum[inline]{How we can measure the effect on the dataset used in the pretraining on each backbone?}
% \input{tables/augmetations_table} 

--


% To shed light on the differences in the predictions on each backbone, we selected a subset of each test set on the benchmarks and apply specific artificial image variations, \ie, Resize, Flip, Grayscale, Color Jitter and Gaussian Blur, to evaluate the zero-shot classification performance on this ``corrupted'' images for each backbone. Figure \ref{wrap-fig:augmentation}, shows the performance variation for each backbone on the intervened images. 
% The results indicate that ResNet 50 and ViT-B-16 are the most resilient to the Flip transformation, RN50x64 is the most resilient to Resize, and RN50x16 is the best for Grayscale. ViT-L-14 and L-14-336 are the most robust for Colour Jitter and Gaussian Blur transformations.  These findings suggest that each backbone has a unique ability to handle specific types of image variations.

--


% Based on these empirical findings, we hypothesize that we can effectively improve the classification performance by learning to combine CLIP backbones. Thus, we propose an approach that is directly inspired by previous work on network calibration, but extended to multiple model combinations. Concretely, our framework can be regarded as a set of variations of Platt scaling \cite{platt1999probabilistic}. In Platt scaling, the logits of a model are used as features for a logistic regression model, which is trained on the validation set to return probabilities. More concretely, given logit scores $\vz_i$ for an example $i$, Platt scaling learns scalar parameters $a, b \in \sR$ and outputs $\hat q_i = \sigma(a \vz_i + b)$ as the calibrated probability. Parameters $a$ and $b$ can be optimized using the NLL loss over the validation set, but during this time, the parameters of the original model are fixed. 

% Since our interest is to combine multiple backbones operating simultaneously in this fashion, our first key insight is to note that Equation \ref{eq:clip_prediction} is essentially equivalent to computing a softmax over a vector of logit-like values $\bar{\vz} \in \sR^{C}$, whose entries are constructed using the inner product between a given input $x$ and the set of labels $\sY$. Concretely, let $\bar{\evz}_c$ denote the c-th entry in vector $\bar{\vz}$, then we define the following.
% \begin{equation}
%     \bar{\evz}_c =  \phi_l(y_c)^\top \phi_v(x) \quad \forall c = [1, \ldots, C]
%     \label{equation:logit-like}
% \end{equation}
% We can use the equation above to rewrite Equation \ref{eq:clip_prediction} simply as $p(y|x) = \text{softmax}(\bar{\vz})$, meaning that we can now essentially equate the output of our zero-shot CLIP classification pipeline, to that of a regular classifier, and interpret the output as a probability distribution over the label space $\sC$.

% We note that a key goal when constructing traditional model ensembles, a technique often used to combine different models, is to increase robustness by increasing the overall confidence of the predictions. In the supervised setting, confidence is generally measured as the probability associated with the predicted label. Though it is expected that a network should provide a calibrated confidence measure in addition to its prediction, it has been shown that deep neural nets are poorly confidence calibrated \cite{guoCalibrationModernNeural2017}. 





% Emulate other backbones by passing the images from the lightweight backbone aiming to improve the performance of the lighted backbone.
% \todonum[inline]{Projection to unify space}
% \todonum[inline]{Rotation matrix found by orthogonal procrustes}
% \todonum[inline]{USE all training dataset using a NN initialized on the rotations with MSE loss}
% \todonum[inline]{USE all training dataset using a NN initialized on the rotations with contrastive loss}
% \todonum[inline]{USE Linear Feature Alignment to close the gap between modalities and then do the same for different backbones in the common space.}

% Once we find a way to emulate other backbones, we aim to unify those predictions/representations.
% \todonum[inline]{Ensembles}
% \todonum[inline]{LinearProbe}
% \todonum[inline]{MoE}
% \todonum[inline]{Calibration}
% \todonum[inline]{Feature Uncertainty}




  %Concretely, \EMT{Chris: please finish explaining this in detail}.
    % we use a genetic algorithm to find the temperatures $T_b$ for each backbone $b 
    % trained Using the training set of the target dataset 




% \paragraph{\textbf{Calibrated confidence} (\CalibratedConfidence)} For this approach, we first calibrate the probabilities of each backbone independently using temperature scaling. Then follow the procedure above and utilize the Shannon entropy of each backbone to select the one with the highest confidence



%These models have extended the paradigm of pre-training to encompass wide-ranging datasets, ranging from hundreds of millions to billions of images. This expansion was significantly influenced by the introduction of Vision Transformers (ViTs) \cite{dosovitskiy2020vit}, which have highlighted the feasibility of training Transformers \cite{NIPS2017_3f5ee243} on such massive datasets within the field of computer vision. Subsequently, various large-scale pre-training methods have surfaced in the domain of computer vision \cite{radford2021learning,yu2022coca,he2022masked}. Among these, a notable category of Vision Foundational Models are exemplified by CLIP~\cite{radford2021learning, schuhmann2022laion, gadre2023datacomp}, which specializes in aligning noisy image-text pairs extracted from web sources. 



%with different architectures. Our current work focuses on studying the differences in image classification among these backbones used to train CLIP.
% There are multiple versions of CLIP trained on different datasets and backbones. Well-studied convolutional backbones like Residual Networks  (ResNet) and ViTs  with different architectures setup. The focus of our current work centers on studying the difference in image classification of each backbone used to train CLIP.


--

\subsection{Combination of Backbones}

% The challenges of effectively fusing different backbones for improved predictions are evident in Figure~\ref{fig:barchar_nnc_zs} (Table~\ref{tab:zs-baselines}). Our experiments aim to compare non-parametric and parametric methods for combining multiple backbones to enhance prediction accuracy. Specifically, we seek to demonstrate the limitations of simple averaging approaches and the efficacy of our proposed method, \NNC{}, in leveraging the strengths of diverse backbones.
In this section, we compare non-parametric and parametric techniques to ensemble CLIP backbones, with no task-specific adaption.
These experiments aim to show the limitations of baseline ensembling methods 
and motivate the adaptive setting of our \NNC{} approach.
Figure~\ref{fig:barchar_nnc_zs} and Table~\ref{tab:zs-baselines} show the performance of each technique.
\textbf{With non-parametric baselines}, 
using the \LogitAvg{} approach consistently fails to enhance the overall performance beyond that of the best backbone. Thus, averaging performance across backbones does not exploit their complementarity, yielding an average delta accuracy of 1.3\%.
%Notably, the \LogitAvg{} approach shows substantial improvement for the \Country{} dataset compared to the best backbone.
When the backbones are calibrated \CLogitAvg{},
performance improves across all datasets except \Gtsrb{}, \Mnist{}, \Resisc45{}, and \SUN397{} compared to the non-calibrated version. Intriguingly, \textbf{Vote T-1} proves ineffective and does not significantly improve accuracy beyond the best backbone.
\textbf{With parametric methods}, we use the training split of each target datasets.
Among these methods, our proposed approach \NNC{} shows
the most substantial improvement over the best backbone, up to $+$35.1\% on the \Eurosat{} dataset. On average, we obtain an improvement of $+$8.1\%
over the \Best{} backbone across datasets.


==> tables/prelim_zs_diffpretrained.tex <==
\begin{table}[tb]
  \caption{Zeroshot accuracy performance of CLIP on \Cifaronehundred{} and \Imagenet{} using different pre-trained datasets LAION-400M (L400M) and LAION-5B (L5B)}
  \label{tab:zs-pretrained}
\centering
    % \resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
    CLIP & \multicolumn{2}{c}{ViT-B-32} & \multicolumn{2}{c}{ViT-B-16} & \multicolumn{2}{c}{ViT-L-14} \\
    Dataset & L400M & L5B & L400M & L5B & L400M & L5B \\
     \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}
    \Cifaronehundred & 67.8 & 75.6 & 71.2 & 76.8 & 77.4 & 83.3 \\
    \Imagenet & 60.2 & 66.6 & 67.1 & 70.2 & 72.7 & 75.2 \\ 
     \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}
\end{tabular}%
% }
\vspace{-0.5cm}
\end{table}

% Datasets paper to take a look
% 1. LAION-400M: Open Dataset of CLIP-Filtered 400 Million Image-Text Pairs https://arxiv.org/abs/2111.02114
% 2. LAION-5B: An open large-scale dataset for training next generation image-text models https://arxiv.org/abs/2210.08402
% 3. DataComp: In search of the next generation of multimodal datasets https://arxiv.org/abs/2304.14108
% 4. Reproducible scaling laws for contrastive language-image learning https://arxiv.org/abs/2212.07143
% 5. DEMYSTIFYING CLIP DATA https://arxiv.org/pdf/2309.16671.pdf
